$F$-wave pairing of cold atoms in optical lattices

The tremendous development of cold atom physics has opened up a whole new opportunity to study novel states of matter which are not easily accessible in solid state systems. Here we propose to realize the $f$-wave pairing superfluidity of spinless fermions in the $p_{x,y}$-orbital bands of the two dimensional honeycomb optical lattices. The non-trivial orbital band structure rather than strong correlation effects gives rise to the unconventional pairing with the nodal lines of the $f$-wave symmetry. With a confining harmonic trap, zero energy Andreev bound states appear around the circular boundary with a six-fold symmetry. The experimental realization and detection of this novel pairing state are feasible.

==> reply_pra.tex <==
Dear Editor,

  We have revised the manuscript according to the suggestions of
the referee and would like to resubmit.

  Referee A agrees with the validity of physics presented in the
previous manuscript, and the importance of our paper in cold 
atom experiments. His suggestion of finite temperate effects
is well-taken. In this revised version, we added one corresponding
paragraph to show the ferromagnetism is robust at temperatures
accessible in experiments. The reply below should convince Referee A 
that our paper is an important breakthrough in cold atom physics.

  We believe that our paper opens up a new important research 
direction for cold atom physics, the itinerant ferromagnetism, 
whose importance comparable to superfluidity/superconductivity. 
Our paper is also helpful for the communication between AMO and 
condensed matter physics. Its high quality meets the high standard
of PRL.

Sincerely,
S. Z. Zhang and C. J. Wu 


**********************************************************
changes made:

1) Typos pointed out by referee A were corrected.

2) According to Referee A's suggestion, we have added a new paragraph 
discussing finite temperature effects with the conclusion that the 
critical temperature (for a finite size optical lattice) is well 
within the experimental reach. 

3) We removed Fig.1 A) in this revised version to save space.
The message conveyed in this figure is already clear in the main text,
thus this  does not cause any confusion.

4) References are being updated. 


*******************************************************************
Reply to referee:


We thank the Referee for his/her positive comments, and his suggestions 
for improving the paper. 

1) Referee's points 1), 2), 4), 5), 7), 9), 10) are comments on typos
and improvning of languages. His points are well-taken. We have followed 
his advice in this new manuscript.


2) Referee's point 3) Physically, with strong enough U, I would expect
that molecules would form out of two particles on the same lattice site 
and occupying the two different orbital states. Then the molecules could 
tunnel between the sites, thus lowering kinetic energy, and one would 
get a bosonic system instead of a fermionic superfluid. There is no 
discussion in the paper as to when this phase is expected to emerge. I
would like to see some discussion of this, especially since the authors 
are suggesting experimental parameters to use for realizing the f-wave 
phase, with a rather large U/t=3 ratio.





-----------------------------------------------------------
1) Referee A states "Yet the aspect of finite temperature - highly 
relevant for current experiments - is not discussed. If the atoms 
occupy a flat band, interaction and chemical potential clearly dominate 
the ground state. How robust are these ordered states at finite 
temperature?". 

We thank Referee A for his very helpful suggestion which is 
well-taken. We have performed both numerical calculation and analytic
estimation for the mean field ferromagnetic critical temperature. 
In this revised version, we added one paragraph stating that the 
ferromagnetic state with the fulfilled flat band is robust
below the temperature scale approximately 1/10 of the on-site 
repulsive interaction, which is experimentally accessible.

The new added paragraph is as follows "We consider the case of the 
filled flat band whose low energy excitations are captured by an 
effective ferromagnetic Heisenberg model defined for plaquette spins, 
and leave the study for the general filling to a future publication. 
In our case, the effective model is defined on a triangular lattice
as $H_{ex}= -J^\prime \sum \vec S_i \cdot \vec S_j$ with $J^\prime 
\approx \frac{U}{18}$. The mean field calculation based on Eq. 2
shows that the critical temperature $T_{mf}$ is at the same order 
of $zJ^\prime/2$ for small values of $U/t_\parallel$ at $\langle 
n \rangle =\frac{1}{2}$ where $z=6$ is the coordination number. 
$T_{mf}$ is the temperature scale for the onset of the nonzero
magnetization of $\vec S$, which is roughly one order smaller than $U$. 
Below $T_{mf}$, the thermal fluctuation of the direction 
of $\vec S$ is described by the $O(3)$ non-linear-$\sigma$ model, 
and no true long range order exits in 2D exists for $T>0$. However, 
the spin correlation length $\xi$ diverges as $\xi/a\approx 
\exp (T_{mf}/T) $ ($a$ is the lattice constant) which can 
easily exceed the small size of the optical lattice (e.g. typically 
$L/a \approx 50$) as $T$ goes smaller than $T_{mf}$. Thus practically 
we can still take $T_{mf}$ as the onset temperature scale of 
ferromagnetism, which is experimentally accessible."

------------------------------------------------------------------
2)Referee A states that `Yet we could not see sufficient reasons to 
recommend publication in the Physical Review Letters. The concept of 
honeycomb optical lattices is by now well known in the field of 
quantum gases (due to refs 16, 17, 18) and the approach to 
ferromagnetism in a flat band provides the expected result."

We thank Referee A for his positive comment on our previous works 
(e.g. refs 16, 17, 18), whose novelty is actually the p-orbital 
physics which is fundamentally different from the well-studied 
graphene physics.

However, we do NOT agree with Referee A's points for his rejection of
this paper. Its scientific importance and the sufficient reasons for 
its publication in PRL are explained as follows.

First, our paper opens up an important new research direction, itinerant 
ferromagnetism, in cold atom physics. As Referee A clearly stated in his 
own report, our proposal is important to realize itinerant ferromagnetism 
with cold atoms, thus is of great interest to cold atom experimentalists. 

As we all agree, itinerant ferromagnetism is one of the central topics 
in contemporary condensed matter physics, whose importance is comparable
to superconductivity/superfluidity. However, in contrast to the extensive 
investigation on fermion superfluidity, ferromagnetism has NOT been paid 
much attention in the cold atom community. The key reason is the 
experimental difficulty, i.e., ferromagnetism usually requires strong 
repulsive interaction which renders the system unstable into dimer 
molecule states. Our proposal nicely solves this problem, and opens 
up a whole new opportunity to investigate itinerant ferromagnetism 
with precise controllability. Furthermore, we also expect 
that our proposal is essential for the investigation of 
spin-dependent transport and even spintronics applications with cold atoms. 

Second, Referee A felt that ferromagnetism through flat band is not surprising,
thus criticized that our work does not have enough reason for the publication 
in PRL. However, we emphasize that the connection between ferromagnetism
and cold atom experiments we proposed is an important breakthrough, thus meets
the high standard of PRL. 

Let us look at an example of a previous milestone work in cold atom physics 
which was also published in PRL, the proposal by Jaksch and Zoller for the 
realization of superfluid/Mott-insulator (SF/MI) transition. Both the 
Bose-Hubbard model they employed and the optical lattice had been 
well-studied in condensed matter and AMO physics respectively, even before 
the cold atom era. The SF/MI transition from Bose-Hubbard model was 
also naturally expected. But the importance of their seminal proposal 
is that they connected two important fields. Similarly, we also hope 
that our work will stimulate a new research direction in cold atom 
physics, i.e, the experimental investigation of ferromagnetism.

Third, in addition to cold atom physics, our work is also important
for the research of ferromagnetism. Due to the intrinsic strong 
coupling nature of ferromagnetism, its mechanism in solid state systems
remains controversial. The flat band ferromagnetism is one of very few 
models whose ground states are exactly solvable. However, most flat band 
models are artificially constructed and difficult to realize in experiments.
Our work provides an experimentally realistic and conceptually natural
flat band ferromagnetism model. 

Furthermore, our investigation goes far beyond the flat band regime by
including various perturbations in realistic experimental systems, 
such as the effects from $\pi$-bonding, p-wave channel interaction, 
extra fillings beyond the flat band, and finite temperature effects. 
These results greatly enriches the research of ferromagnetism.

In summary, our paper proposed a ferromagnetic systems with cold atoms
with unprecedented experimental controllability. It greatly benefits 
both fields of cold atom physics and condensed matter physics.

--------------------------------------------------------------------
3) We thank Referee A for his pointing several typos in the paper.
We have already corrected them.













